Dual-high-frequency VLBI study of blazar-jet brightness-temperature gradients and collimation profiles

On the kiloparsec scale, extragalactic radio jets show two distinct morphologies related to their power: collimated high-power jets ending in a bright termination shock and low-power jets opening up close to the core and showing a more diffuse surface brightness distribution. The emergence of this morphological dichotomy on the parsec scale at the innermost jet regions can be studied with very-long-baseline interferometry (VLBI) radio observations of blazars in which the jet emission is strongly Doppler boosted due to relativistic bulk motion at small angles between the jet direction and the line of sight. We seek to characterize the geometry and emission profiles of the parsec-scale radio jets of flat-spectrum radio quasars (FSRQs) and BL Lacertae objects (BL Lacs) on parsec scales to derive properties of the magnetic field, environment, and energetics for different classes of extragalactic jets. We analyze the VLBI radio data of 15 FSRQs, 11 BL Lacs, and two radio galaxies contained in both the MOJAVE data archive and the Boston University BU blazar group sample archive at 15 GHz and 43 GHz, repectively. We derived the brightness-temperature and jet-width gradients along the jet axis from parameterizations of the jets using 2D Gaussian brightness distributions. In most BL Lac objects, the diameter and brightness-temperature gradients along the jet axis can generally be described well by single power laws, while the jets of FSRQs show more complex behavior and remain more strongly collimated on larger physical scales. We find evidence for a transition of the global jet geometry from a parabolic to a conical shape in the BL Lac objects 3C 66A, Mrk 421 and BL Lacertae, the radio galaxy 3C 111 and the FSRQs CTA 26, PKS 0528+134,4 C +71.07,4C +29.45, and 3C 279 outside the Bondi sphere.

==> magnetic_field.tex <==
\section{Magnetic field in the radio cores}
\label{magnetic_field}
Following \citet{baczko2016} we calculate the magnetic field in the core region of the jets, since this is the region where the emssion transitions from optically thick to optically thin, via synchrotron cooling, however in this case, due to relativistic bulk velocities, beaming effects and small inclination angles, certain adjustments have to be taken into account.\newline
\subsection{Deriviation}
According to \citet{rybicki_lightman_1979}, the emitted power of an electron with a random pitch-angle distribution is given by 
\begin{equation}
P = \frac{4}{3}\, \sigma _T \,c \,\beta _e ^ 2 \, \gamma ^2 \, u_B
\end{equation}
Where $c$ is the speed of light, $u_B=\frac{B^2}{8\pi}$ is the magnetic field density, $\sigma _T = \frac{8\pi \, r_0 ^2}{3}$ is the Thomson cross section, defined by the classical electron radius $r_0$ and $\beta _e$ is the electron velocity. To obtain the cooling time of the electron, the energy loss has to be calculated

\begin{equation}
\dot{E} _{\mathrm{loss}} = -P \, \rightarrow \, \frac{\mathrm{d}\gamma}{\mathrm{d}t} = -\frac{P}{m_e\, c^2}\, = - \frac{4}{3}\, \frac{\sigma _T}{m_e\,c}  \,\beta _e ^ 2 \, \gamma ^2 \, u_B\, .
\end{equation}

Separating the variables leads to 
\begin{equation}
\frac{\mathrm{d}\gamma}{\gamma ^2} = -\frac{4}{3}\, \frac{\sigma _T}{m_e\,c} \,\beta _e ^2  \, u_B \,\mathrm{d}t\, ,
\end{equation}
integration yields
\begin{equation}
-\frac{1}{\gamma} = -\frac{4}{3}\, \frac{\sigma _T}{m_e\,c} \,\beta _e ^2  \, u_B t_c\, .
\end{equation}
The cooling time of the electron $t_c$ then reads
\begin{equation}
t_c =  \frac{3}{4}\, \frac{m_e \, c}{\sigma _T\, \beta _e ^2 \, u_B \, \gamma}
\end{equation}
Inserting the magnetic field density and expressing the Lorentz factor $gamma$ via the critical frequency, where the optical depth $\tau = 1$, 
\begin{equation}
\nu _c = \frac{3}{4\pi}\, \frac{e\,B}{m_e \, c} \, \gamma^2 \, \rightarrow \, \gamma = \sqrt{\frac{4\pi \, m_e \, c\, \nu _c}{3\, e \, B}}\, ,
\end{equation}
the cooling time then reads 
\begin{equation}
t_c = \frac{3}{4}\, \frac{m_e \, c}{\sigma _T\, \beta _e ^2\, \frac{B^2}{8\pi}} \sqrt{\frac{3\, e \, B}{4\pi \, m_e \, c \, \nu _c}} = 3\sqrt{3\pi} \, \sqrt{\frac{m_e \, c \, e }{\nu _c}} \, \frac{B^{-\frac{3}{2}}}{\sigma _T \, \beta _e ^2}
\end{equation}
Since the electron moves in a bulk which itself moves at highly relativistic speeds with a bulk Lorentz factor of $\Gamma$, the cooling time becomes larger due to time dilatation. Furthermore, due to relativistic beaming, the critical frequency has to be corrected with the Doppler factor $\delta = \frac{1}{\Gamma(1-\beta _{b,\mathrm{int}}\mathrm{cos}(\theta))} $, where $\theta$ is the inclination angle, under which the emission of the moving bulk is observed and $\beta _{b,\mathrm{int}}$ is the intrinsic velocity of the bulk.
\begin{equation}
\begin{gathered} 
\label{cooling_time}
t_c \rightarrow t_c ' = \Gamma \, t_c;\, \nu _c \rightarrow \nu_c ' = \frac{\nu _c}{\Gamma} \\
t_c = \Gamma\,  3\sqrt{3\pi} \, \sqrt{\frac{m_e \, c \, e\, \delta }{\nu _c}} \, \frac{B^{-\frac{3}{2}}}{\sigma _T \, \beta _e ^2} \, \text{(observables in observer's frame)}
\end{gathered}
\end{equation}

The projected distance over which the electrons pass while cooling at an optical depth of unity should then equal the size of the core region in the VLBI images $t_c = \frac{d_{CR}}{\beta _e}$. This in turn has to be de-projected, since blazars have small angles to the line of sight. One can assume that the electrons travel nearly at the speed of light, meaning $\beta _e \rightarrow 1$. Therefore Eq.\ref{cooling_time} can be reorganized, expressing the magnetic field as
\begin{equation}
\begin{gathered} 
\label{B_cooling}
t_c = \frac{d_{CR}}{c}\, (\beta _e \rightarrow 1),\, d_{CR} \rightarrow d_{CR} ' = \frac{d_{CR}}{\mathrm{sin}(\theta)} \, \text(de-projected) \\
B = \left(\frac{d_{CR}\, \sigma _T}{3\sqrt{3\pi}\, \Gamma \, \mathrm{sin}(\theta)}\, \sqrt{\frac{\nu _c}{m_e \, c \, \delta }}\right)^{-\frac{2}{3}};\, [B] = \mathrm{G},\, [d_{CR}] = \mathrm{cm}
\end{gathered}
\end{equation}
\subsection{Concerning the intrinsic bulk speed, the bulk Lorentz factor and the maximum apparent jet speed}
In Eq.\ref{B_cooling} the bulk Lorentz factor $\Gamma$ itself and the Doppler factor $\delta$ with the Lorentz factor within, and the intrinsic bulk speed, appear. If the maximum apparent speed in a jet is sufficiently large, the bulk Lorentz factor can be estimated by this speed, the error occurring at this point is smaller, the larger the intrinsic speed of the jet is. At $\sim 90\%$ of the speed of light, the error, done by this method is $\sim 10\%$. One also has to take account that this statement is done under the assumption of a critical inclination angle, where the apparent speed of the jet peaks. When taking a sample of radio loud AGN, and drawing a random source, the chance, finding a blazar under the critical angle is about $50\%$, see \citet{cohen2007}. For the purposes of the B-field calculation it is assumed that the approximation $\Gamma \sim \beta _{\mathrm{b,max,app}}$ to be valid. Eq.\ref{B_cooling} then reads.
\begin{equation}
\begin{gathered}
\label{B_approx}
\Gamma \rightarrow \beta _{\mathrm{b,max,app}} \\
B = \left(\frac{d_{CR}\, \sigma _T}{3\sqrt{3\pi}\, \beta _{\mathrm{b,max,app}} \, \mathrm{sin}(\theta)}\, \sqrt{\frac{\nu _c}{m_e \, c \, \delta }}\right)^{-\frac{2}{3}} \\
[B] = \mathrm{G},\, [d_{CR}] = \mathrm{cm},\, [\beta _{\mathrm{b,max,app}}] = \mathrm{cm}/\mathrm{s}\, .
\end{gathered}
\end{equation}
This of course is also applied for the Doppler factor $\delta$.

\subsection{problematic sources}
For sources where no luminosity distance is given, the magnetic field in the radio core cannot be calculated, since the size of the region where the electrons pass through has to be available in cm and the apparent maximum jet speed in cm/s. Furthermore, for sources, where the maximum apparent speed is very low ($\beta _{\mathrm{app,max}}<1$), this method cannot be applied.

\subsection{The scaling of the magnetic field}
The absolute position of the radio cores with respect to the jet engine is not known due to the use of the closure relations in the imaging process which destroys the absolute phase information, \citet{jennison1958}. Also it is not clear where - with respect to the position of host galaxies's SMBH, which is also often not known - the position of the radio core ($\tau \sim 1$) is located. Therefore the scaling of the calculated core magnetic field is arbitrary. However utilizing different ideas of magnetic fields in the SMBH's ergospheres, estimates of the scales of distances between the magnetic fields in the supposed ergosphere and the magnetic field in the radio cores can be calculated.
 The scaling of the magnetic field from the ergosphere to the radio core is assumed to follow a power law like:
 \begin{equation}
 \begin{gathered}
 \label{ergosphere_scaled}
 B_{c,\nu} =  B_{\mathrm{ergosphere}}  \: r_\nu ^{-b}\\
 r_{\nu} =\left( \frac{B_{\mathrm{ergosphere}}}{B_{\nu}} \right)^{\frac{1}{b}}\: .\\
 \end{gathered}
 \end{equation}

In the following, two different cases, describing $B_{\mathrm{ergosphere}}$ are studied. The first cases assumes that the magnetic field strength in the ergosphere nears the Eddington field as given by \citet{daly2009}, \citet{daly2011} and \citet{daly2014}:

\begin{equation}
\label{B_edd_daly}
\frac{B_{\mathrm{Eddington}}}{10^4} \, G = 6\times \left(\frac{M}{10^8 M_\odot}\right)^{-\frac{1}{2}} 
\end{equation}

Secondly we assume that the jet is driven by the \citet{blandford_znajek} process. In this case a polodial magnetic field component, driven by the spin of the black hole supports a jet with a certain luminosity. \citet{daly2014} show the formula for the polodial magnetic field component
\begin{equation}
\frac{B_{\mathrm{Blandford-Znajek}}}{10^4 \, G} =  \left( \frac{P_j}{10^{44}}\right)^{0.5} \left(\frac{M}{10^8}\right)^{-1} \frac{\sqrt{5}}{j}
\end{equation}

In both cases the black hole masses need to be known. The black hole masses are taken from \citet{zhou2008}. For sources in the sample, where no mass is given, the mean mass of the represented sources is taken ($\mathrm{log}(M/M_{\odot})\sim 8.77$). This can be done without risking too much systematic errors, because the masses of the black holes usually have errors, spanning an order of magnitude or more, however the impact of this assumption will be discussed separately when analyzing the results from these calculations.\newline 
In the second case, the spin paramrter is set to $j=0.5$ which of course will not yield absolute positions, however supposed relative distances within the source classes will still show. This is a reasonable guess, since in radio galaxies spin parameters range between $0.1\lesssim j \lesssim 0.99$ are found, see \citet{daly2014}. 
The jet powers $P_j$ are obtained by estimating the power budget of the extended, un-beamed emission in the manner of \citet{godfrey2013}. For this the luminosities of the extended emission is obtained for each of the sources from \citet{Kharb2010}. 
The jet powers, under the assumption, FSRQs can be associated with rotated FR2 galaxies and BL Lacs with FR1 galaxies (CITE ANY UNIFICATION PAPER), can be estimated according to 
\begin{equation}
\begin{gathered}
P_{j,\mathrm{FSRQs}} = 3 \times 10^{44} \left(\frac{L_{151}}{10^{25}}\right)^{0.67} \, W \\
P_{j,\mathrm{BLLacs}} = 5 \times 10^{44} \left(\frac{L_{151}}{10^{25}}\right)^{0.64} \, W
\end{gathered}
\end{equation}
In \citet{Kharb2010}, the luminosities are measured at $1.4\,\mathrm{GHz}$, the method from \citet{godfrey2013} measures at $0.151\,\mathrm{GHz}$, therefore the Flux is sacled to the needed frequency with a power law of $\alpha \sim -0.75$ due to the steepened spectrum of the extended, un-beamed emission of blazars at these frequencies.\newline
Table \ref{tab_B} summarizes the parameters, used to obtain the different magnetic fields in the ergosphere, as well as the calculated magnetic fields in the radio cores at the respective frequencies.
For each source four scenarios can be tested now. In any case a poloidal scaling behavior is assumed between the ergosphere and the radio core ($d\propto R^{-2}$). For each magnetic field model (Blandford-Znajek and Eddington), two jet-geometry cases are studied. First we assume that the scaling behavior of the diameter, found in the VLBI jets, extends to the ergosphere, meaning ($B\propto R^{-2}$, $R\propto r^l\rightarrow B\propto r^{-2\times l}$, \textbf{scenario A}). The other case describes a jet which expands freely after the initial collimation and acceleration with a conical geometry ($l=1$) whereupon a recollimation is triggered near the radio core (the process itself if no concern here), leading to the measured, mostly collimated ($l<1$), measured geometries (\textbf{scenario B}). In this case the poloidal magnetic field of course scales like $B\propto r^{-2}$. The distance for any of those four cases is calculated according to Eq.\ref{ergosphere_scaled}, while the results are summarized in Tabs.\ref{tab_B_scaling} and \ref{tab_B_scaling2} and illustrated in Figs.\ref{B_edd_plots} and \ref{B_edd_plots2}.
Figure \ref{B_edd_plots} shows the results including sources where the black hole mass was guessed ($\mathrm{log}\left(\frac{M}{M_{\odot}}\right)=8.77$), while Fig.\ref{B_edd_plots2} excludes those cases. 

The scales for d range between $5\times 10^1\lesssim d/r_g \lesssim 10^3$. Disregarding the FSRQs where the magnetic field scaling is determined by the measured geometry (red data points) and only taking into account the conical assumed FSRQs (orange) and BL Lac objects in both geometries (blue,cyan), the distances between the ergosphere and the respective radio cores scale between $ 50 \lesssim d/r_g \lesssim 10^3$.\newline
In the case of NGC 1052 where absolute distances can be measured due to the source being relatively near ($D_l \sim 20 \mathrm{Mpc}$) and the inclination angle being large ($60\lesssim \vartheta / \mathrm{deg} \lesssim 90$), the position along the jet axis where the scaling of the magnetic field switches form polodial to torodial is located at around $50r_g$, see \citet{baczko2016}.\newline
The model applied here describes a scenario where the poloidal magnetic field component drives the jet from the ergosphere after switching to a toroidal behavior.\newline
 This torodial behavior is measured within the VLBI jets in the equipartition case in Subsec.\ref{subsec_b_gradients} for all sources within the errors. This scenario is reasonably comparable to the case of NGC 1052 when interpreting the distances between the ergospheres and the radio cores with the point where the magnetic fields change the behavior from poloidal to toroidal.\newline  
The FSRQs, where the measured geometry determines magnetic field scaling suggest that the radio cores are extremely near to the ergosphere $ 10^{-3} \lesssim d/r_g \lesssim 10 r_g$. This seems unphysical with respect to the discussion above and might hint to a scenario where at least one break in the scaling of the diameter scaling of the jet is present. A change of the diameter scaling is not uncommon and can also be observed and studied in this sample, e.g. in the case of BL Lac, see also \citet{Kovalev2019}. However as also argued by \citet{Kovalev2019}, the spatial resolution has to be small enough to observe this at small scales. for a fixed maximum baseline length and observing frequency this means that sources where this can be observed tend to need small redshifts $(z\ll1)$.
A change in the diameter scaling behavior is also observed in M87 where the scaling changes from  about $d\propto r^{\sim 0.58}$ to $d \propto r^{\sim 1}$ at the position of the Bondi radius to ($2.5\times 10^{5} r_g$), see \citet{nakamura2013}, which they interpret as the beginning of a magnetic nozzle.\newline
Considering this discussion, we assume the FSRQs to yield unphysical results in the case of scenario A, however in the following it will be studied whether there is a measurable difference between any of the classes, defined in the plots. When including sources with guessed black hole masses, the overall trends seem not to be affected. Especially BL Lacs in the regime $d\sim 10 r_g$ are affected besides the RGs.  However since there are no RGs with measured black hole masses it is impossible to test whether true systematic trends are seen or not when including those. This is why sources with guessed black hole masses are excluded from the further discussion regarding systematic differences within the sources.\newline
A KS test is performed in the sample with the measured black hole masses to check whether differences can be measured between the different subclasses defined in the plot. In the case where the measured geometry determined the magnetic field's scaling, the KS test yields $d_{CDF}\sim 0.74$ with $p\sim 2.7\times 10^{-5}$ when comparing FSRQs (red and orange data points for both frequencies) with BL Lacs (blue and cyan data points for both frequencies). In the case of a forced conical geometry the KS test yields $d_{CDF}\sim 0.76\; ,p\sim 1.6\times 10^{-5}$. Both cases suggest that there is a systematic difference between those source classes when comparing the model dependent distances between the ergosphere and the respective radio core.\newline
Comparing the scenarios A and B for the FSRQs (red and orange data points), the KS test yields  $d_{CDF}\sim 0.825$ with $p\sim 5\times 10^{-13}$, suggesting that the underlying distribution function for these values is different. As discussed above, we consider scenario A for the FSRQs as unphysical, which also substantiated by the statistical analysis. Therefore it can be assumed that scenario B holds for FSRQs.
Comparing the scenarios A and B for BL Lacs (blue and cyan) data points, the KS test yields $d_{CDF}\sim 0.5$ with $p\sim 5\times 6.6\%$. In this case it is not clear whehter the underlying distribution functions differ or not, therefore we do not exclude any of the scenarios for BL Lacs. Figure \ref{B_edd_physical} shows the plot with the data points we consider as physically reasonable solutions when interpreting the distance between the ergosphere and the respective radio cores as the point where the scaling of the magnetic field changes from poloidal to toroidal in the sense of the discussion above. 
FSRQs have a higher accretion flow and thus higher particle densities on the scales of the ergosphere and beyond (BH -corona?) than BL Lacs, see \citet{mondal2019}. This could explain that the region where the poloidal magnetic field dominates is clinched with respect to BL Lac object where the evolution is not hindered. The jet of the FSRQ has to plow through this matter and at a certain point (near the measured radio cores) the conical expanding jet recollimates and changes its magnetic field scaling behavior to toroidal, which in turn enables the jet to self-collimate up to large scales. This interaction with the higher particle density could also lead to shear layers within the jet, producing different velocities in the jet layers along the jet axis which in turn can produce shocks, manifesting in knots which are often seen in FSRQs. BL Lacs show lower accretion flow, indicating a smaller particle density. This in turn can explain why the poloidal magnetic field component holds up to larger scales before turning toroidal, being able to self-collimate a jet which also explains why FSRQs tend to show higher collimations than BL Lacs.






%To scale the magnetic fields with the given power laws, derived in Sec.\ref{subsec_b_gradients}, a distinguished point along the jet axis where the diameters of the $15\,\mathrm{GHz}$ and $43\,\mathrm{GHz}$ jets are equal, can be calculated with the model, illustrated in Fig.\ref{jet_model_15_43}.

%\begin{figure}
%\centering
%	\includegraphics[width=\hsize]{./jet_model/jet_modell.pdf}

%      \caption{The red and blue curve depict the jet at $15\,\mathrm{GHz}$ and $43\,\mathrm{GHz}$, respectively. The ocmponents A and C depict the unresolved radio cores while the components B and D show the first resolved component at the given frequencies. }
%\label{jet_model_15_43}
%\end{figure}

%\begin{equation}
%\begin{gathered} 
%\label{B_sc_system}
%% d_{0,15} = d_{15} (r_{15}-r'_{15})^{l_{15}}\: (\mathrm{I})\\
% d_{0,43} = d_{43} (r_{43}-r'_{43})^{l_{43}}\: (\mathrm{II})\\
%(\mathrm{I}) = (\mathrm{II})\\
%\rightarrow  \frac{d_{15}}{d_{43}} = \frac{(r_{43}-r'_{43})^{l_{43}}}{(r_{15}-r'_{15})^{l_{15}}}\: (\mathrm{III})\\
%\text{Model: Let the diameter at the jet base at 43 GHz be $10r_g$}\\
%\rightarrow
%10r_g=d_{43} (r_{43} - r'_{43})^{l_{43}}\\
%\frac{10r_g}{d_{43}} = (r_{43} - r'_{43})^{l_{43}}\: (\mathrm{IV})\\
%r_{43} = r'_{43} + \left(\frac{10r_g}{d_{43}}\right)^{\frac{1}{l_{43}}}\: (\mathrm{V})\\
%\mathrm{IV}\text{ in } \mathrm{III}\\
%\rightarrow \frac{d_{15}}{d_{43}} = \frac{10r_g}{d_{43}(r_{15}-r'_{15})^{l_{15}}}\\
%r_{15} = r'_{15} + \left(\frac{10r_g}{d_{15}}\right)^{\frac{1}{l_{15}}}\: (\mathrm{VI})\\
%\end{gathered}
%\end{equation}
 %The subscripts $15$ and $43$ refer to the frequencies ,  $d_{0,\nu}$ is the diameter of the jet at a given frequency and point along the jet axis $d_{\nu}$ is the diameter of the first resolved component in a given image. This was obtianed for each source by finding the first resolved component in each epoch and taking the mean value out of the diameters. The first resolved component is usually the second brightest after the unresolved core and also the closest to the core. Bright knots in FSRQs can deviate here in the sense that the knots can become very high in flux, therefore a cautious filtering here is needed. The distance of the unresolved radio core from the point where the jets have the same diamter $r_\nu$ has to be shifted by the position of the first resolved component $r'_\nu$. The magnetic field can be scaled according to



%To get $r_\nu$ in terms of teh gravitation radius $r_g$... Here the black hole masses need to be known. The black hole masses are taken from \citet{zhou2008}. For sources in the smaple, where no mass is given, the mean mass of the represented sources is taken ($\mathrm{log}(M/M_{\odot})\sim 8.77$). This can be done without risking too much systematic errors, because the masses of the black holes usually have errors, spanning an order of magnitude or more, however the impact of this assumption will be discussed separately when analyzing the results from these calculations.
%The results of the calculations are summarized in Tab.\ref{tab_B}. The results of the $B$-field calculation and scaling are listen in Tab.\ref{tab_B}.

\iffalse
\begin{table*}
\caption{\textbf{col.1}: name and class; \textbf{col.2}: black hole mass; \textbf{col.3}: estimated jet powers from the extended unbeamed emission; \textbf{col.4}: estimated magnetic field in the $15\,\mathrm{GHz}$ radio core due to synchrotron cooling; \textbf{col.5}: estimated magnetic field in the $43\,\mathrm{GHz}$ radio core due to synchrotron cooling; \textbf{col.6}: Eddington magnetic field strength of the SMBH ; \textbf{col.7}: polodial magnetic field component assuming a Blandford-Znajek driven jet with a spin parameter of j=0.5}
\label{tab_B}
\begin{tabular}{lcccccc}
\toprule
B1950, class& $\mathrm{log}\left(\frac{M}{M_{\odot}}\right)$& $P_j\, \frac{\mathrm{erg}}{s}$ & $B_{c,15}/G$ &$B_{c,43}/G$&$B_{\mathrm{eddington}}/G$&$B_{\mathrm{Blandford-Znajek},j=0.5}/G$\\
\midrule
0219+428 B & 8.77 & 2.16E+45 & 1.77 & 1.46 & 2.47E+04 & 3.53E+04 \\ \midrule
0336$-$019 Q & 8.78 & 8.21E+46 & 0.69 & 1.2 & 2.44E+04 & 2.13E+05 \\ \midrule
0415+379 G & 8.77 & 3.15E+46 & 3.33 & 3.36 & 2.47E+04 & 1.35E+05 \\ \midrule
0430+052 G & 8.77 & 2.78E+45 & 1.99 & 3.88 & 2.47E+04 & 4.00E+04 \\ \midrule
0528+134 Q & 8.77 & 1.73E+47 & 0.71 & 1.49 & 2.47E+04 & 3.16E+05 \\ \midrule
0716+714 B & 8.77 & 3.74E+46 & - & - & - & -\\ \midrule
0735+178 B & 8.77 & 2.58E+46 & - & - & - & -\\ \midrule
0827+243 Q & 8.77 & 8.84E+46 & 1.01 & 1.17 & 2.47E+04 & 2.26E+05 \\ \midrule
0829+046 B & 8.49 & 3.04E+46 & 0.97 & 1.42 & 3.41E+04 & 2.52E+05 \\ \midrule
0836+710 Q & 9.49 & 2.11E+47 & 0.82 & 1.13 & 1.08E+04 & 6.64E+04 \\ \midrule
0851+202 B & 8.77 & 1.14E+46 & 1.86 & 1.97 & 2.47E+04 & 8.11E+04 \\ \midrule
0954+658 B & 8.77 & 2.16E+45 & - & - & - & -\\ \midrule
1101+384 B & 8.77 & 2.16E+45 & - & - & - & -\\ \midrule
1127-145 Q & 9.18 & 1.05E+47 & 0.49 & 0.92 & 1.54E+04 & 9.58E+04 \\ \midrule
1156+295 Q & 9.19 & 1.45E+47 & 1.3 & 2.04 & 1.52E+04 & 1.10E+05 \\ \midrule
1219+285 B & 8.77 & 2.16E+45 & 2.07 & 2.0 & 2.47E+04 & 3.53E+04 \\ \midrule
1222+216 Q & 8.77 & 2.26E+47 & 2.52 & 2.27 & 2.47E+04 & 3.61E+05 \\ \midrule
1226+023 Q & 8.76 & 4.69E+47 & 0.89 & 1.8 & 2.50E+04 & 5.32E+05 \\ \midrule
1253$-$055 Q & 8.53 & 6.18E+47 & 0.99 & 1.22 & 3.26E+04 & 1.04E+06 \\ \midrule
1308+326 Q & 8.77 & 9.52E+46 & 1.46 & 1.47 & 2.47E+04 & 2.34E+05 \\ \midrule
1633+382 Q & 10.14 & 1.04E+47 & 1.37 & 2.01 & 5.11E+03 & 1.04E+04 \\ \midrule
1652+398 B & 8.77 & 2.16E+45 & - & - & - & -\\ \midrule
1730-130 Q & 8.77 & 3.36E+47 & 1.23 & 1.38 & 2.47E+04 & 4.40E+05 \\ \midrule
1749+096 B & 8.34 & 7.19E+45 & 1.78 & 1.69 & 4.06E+04 & 1.73E+05 \\ \midrule
2200+420 B & 8.42 & 2.16E+45 & 14.78 & 4.59 & 3.70E+04 & 7.91E+04 \\ \midrule
2223-052 Q & 8.54 & 1.61E+47 & 0.58 & 0.69 & 3.22E+04 & 5.17E+05 \\ \midrule
2230+114 Q & 8.64 & 1.65E+47 & 0.75 & 1.0 & 2.87E+04 & 4.16E+05 \\ \midrule
2251+158 Q & 8.87 & 4.30E+47 & 0.51 & 0.99 & 2.20E+04 & 3.96E+05 \\ \bottomrule
\end{tabular}
\end{table*}



\begin{table*}
\caption{\textbf{col.1}: name and class;\textbf{col.2}: scaling power of the polodial magnetic field component with a given geometry ; \textbf{col.3}: distance between the location of $B_{\mathrm{eddington}}$ and $B_c$ along the jet axis with the measured geometry; \textbf{col.4}: distance between the location of $B_{\mathrm{Blandford-Znajek},j=0.5}$ and $B_c$ along the jet axis with the measured geometry ; \textbf{col.5}: distance between the location of $B_{\mathrm{eddington}}$ and $B_c$ along the jet axis with the a conical geometry ; \textbf{col.6}: distance between the location of $B_{\mathrm{Blandford-Znajek},j=0.5}$ and $B_c$ along the jet axis with a conical geometry; Remark: the first line of each source block gives the data for $15\, \mathrm{GHz}$, the bottom line the data for $15\, \mathrm{GHz}$.}
\label{tab_B_scaling}
\begin{tabular}{lccccc}
\toprule
B1950, class& $b=-2\times l$ & $d_{\mathrm{geo,ed}}/r_g$& $d_{\mathrm{geo,bz}}/r_g$& $d_{\mathrm{conus,ed}}/r_g$& $d_{\mathrm{conus,bz}}/r_g$\\
\midrule

0219+428 B & -1.29 & 2.20E+01 & 1.67E+01 & 3.00E+02 & 2.51E+02 \\
  & -1.16 & 8.13E+00 & 5.98E+00 & 2.73E+02 & 2.28E+02 \\ \midrule
0336-019 Q & -1.12 & 3.09E+00 & 4.50E-01 & 1.85E+02 & 6.26E+01 \\
  & -1.45 & 3.75E+01 & 8.46E+00 & 2.43E+02 & 8.25E+01 \\ \midrule
0415+379 G & -1.24 & 2.66E+01 & 6.75E+00 & 4.12E+02 & 1.76E+02 \\
  & -1.18 & 1.86E+01 & 4.41E+00 & 4.13E+02 & 1.77E+02 \\ \midrule
0430+052 G & -1.22 & 1.60E+01 & 1.08E+01 & 3.18E+02 & 2.50E+02 \\
  & -1.04 & 7.52E+00 & 4.72E+00 & 4.45E+02 & 3.49E+02 \\ \midrule
0528+134 Q & -1.41 & 2.14E+01 & 3.51E+00 & 1.90E+02 & 5.31E+01 \\
  & -1.18 & 9.68E+00 & 1.13E+00 & 2.75E+02 & 7.71E+01 \\ \midrule
0716+714 B & - & - & - & - & - \\ \midrule
0735+178 B & - & - & - & - & - \\ \midrule
0827+243 Q & -1.48 & 3.83E+01 & 8.58E+00 & 2.27E+02 & 7.52E+01 \\
  & -0.98 & 1.35E+00 & 1.40E-01 & 2.44E+02 & 8.09E+01 \\ \midrule
0829+046 B & -1.6 & 9.73E+01 & 2.79E+01 & 3.60E+02 & 1.32E+02 \\
  & -1.49 & 7.82E+01 & 2.05E+01 & 4.36E+02 & 1.60E+02 \\ \midrule
0836+710 Q & -1.75 & 2.97E+01 & 1.05E+01 & 5.90E+01 & 2.38E+01 \\
  & -0.95 & 4.20E-01 & 6.16E-02 & 6.93E+01 & 2.79E+01 \\ \midrule
0851+202 B & -1.35 & 3.15E+01 & 1.31E+01 & 3.08E+02 & 1.70E+02 \\
  & -2.13 & 4.21E+02 & 2.41E+02 & 3.17E+02 & 1.75E+02 \\ \midrule
0954+658 B & - & - & - & - & - \\ \midrule
1101+384 B & - & - & - & - & - \\ \midrule
1127-145 Q & -0.71 & 6.47E-03 & 4.95E-04 & 7.80E+01 & 3.13E+01 \\
  & -0.96 & 5.52E-01 & 8.25E-02 & 1.06E+02 & 4.27E+01 \\ \midrule
1156+295 Q & -1.11 & 2.96E+00 & 5.01E-01 & 1.25E+02 & 4.64E+01 \\
  & -1.05 & 2.66E+00 & 4.03E-01 & 1.56E+02 & 5.82E+01 \\ \midrule
1219+285 B & -1.83 & 2.10E+02 & 1.73E+02 & 3.24E+02 & 2.71E+02 \\
  & -1.06 & 4.78E+00 & 3.41E+00 & 3.19E+02 & 2.67E+02 \\ \midrule
1222+216 Q & -1.96 & 3.26E+02 & 8.30E+01 & 3.58E+02 & 9.37E+01 \\
  & -1.37 & 4.02E+01 & 5.69E+00 & 3.40E+02 & 8.89E+01 \\ \midrule
1226+023 Q & -1.44 & 2.88E+01 & 3.42E+00 & 2.16E+02 & 4.69E+01 \\
  & -0.9 & 9.46E-01 & 3.21E-02 & 3.08E+02 & 6.67E+01 \\ \midrule
1253-055 Q & -1.75 & 1.65E+02 & 2.29E+01 & 3.40E+02 & 6.03E+01 \\
  & -1.21 & 1.37E+01 & 7.90E-01 & 3.77E+02 & 6.68E+01 \\ \midrule
1308+326 Q & -1.33 & 2.32E+01 & 4.27E+00 & 2.72E+02 & 8.84E+01 \\
  & -1.62 & 8.62E+01 & 2.14E+01 & 2.74E+02 & 8.89E+01 \\ \midrule
1633+382 Q & -1.25 & 2.13E+00 & 1.20E+00 & 2.48E+01 & 1.73E+01 \\
  & -1.54 & 9.19E+00 & 5.77E+00 & 3.00E+01 & 2.10E+01 \\ \midrule
1652+398 B & - & - & - & - & - \\ \bottomrule


\end{tabular}
\end{table*}



\begin{table*}
\caption{continuation of Tab.\ref{tab_B_scaling}}
\label{tab_B_scaling2}
\begin{tabular}{lccccc}
\toprule
B1950, class& $b=-2\times l$ & $d_{\mathrm{geo,ed}}/r_g$& $d_{\mathrm{geo,bz}}/r_g$& $d_{\mathrm{conus,ed}}/r_g$& $d_{\mathrm{conus,bz}}/r_g$\\
\midrule
1730-130 Q & -1.67 & 9.30E+01 & 1.65E+01 & 2.50E+02 & 5.94E+01 \\
  & -1.68 & 1.03E+02 & 1.86E+01 & 2.65E+02 & 6.27E+01 \\ \midrule
1749+096 B & -1.92 & 5.13E+02 & 2.41E+02 & 6.33E+02 & 3.06E+02 \\
  & -1.19 & 2.02E+01 & 5.96E+00 & 6.16E+02 & 2.98E+02 \\ \midrule
2200+420 B & -1.7 & 7.96E+02 & 5.09E+02 & 1.59E+03 & 1.09E+03 \\
  & -1.85 & 6.21E+02 & 4.13E+02 & 8.84E+02 & 6.05E+02 \\ \midrule
2223-052 Q & -1.58 & 5.94E+01 & 1.02E+01 & 2.55E+02 & 6.37E+01 \\
  & -1.29 & 1.43E+01 & 1.66E+00 & 2.78E+02 & 6.94E+01 \\ \midrule
2230+114 Q & -1.27 & 1.21E+01 & 1.48E+00 & 2.44E+02 & 6.42E+01 \\
  & -1.04 & 2.37E+00 & 1.79E-01 & 2.83E+02 & 7.43E+01 \\ \midrule
2251+158 Q & -1.67 & 4.72E+01 & 8.38E+00 & 1.36E+02 & 3.20E+01 \\
  & -0.87 & 2.83E-01 & 1.02E-02 & 1.89E+02 & 4.46E+01 \\ \bottomrule

\end{tabular}
\end{table*}
\fi

\begin{figure}
\centering
  \includegraphics[width=\hsize]{./B_edd_plots/B_sc_tot.pdf}
  %\includegraphics[width=\hsize]{./B_edd_plots/B_sc_prog.pdf}
  %\includegraphics[width=\hsize]{./B_edd_plots/B_Maldacenasc_schwarzschild.pdf}
  %\includegraphics[width=\hsize]{./B_edd_plots/B_sc_retr.pdf}
      \caption{The distance between the core region of the radio jet with the calculated magnetic field and the position along the jet axis where a polodial component of the magnetic field in the ergosphere accelerates a jet is plotted for two cases in gravitation radii ($r_g$) against the magnetic field in the core in $B_c$. One case is calculated for a given Eddington magnetic field strength, the other case is the magnetic field for a Blandford-Znajek driven jet with the estimated jet powers and black hole masses from Tab.\ref{tab_B} and a spin parameter of j=0.5.
      The classes are distinguished as follows: \textbf{Blue}: BL Lac for the measured geometry in the Eddington field case at $15\, \mathrm{GHz}$ (crosses) and $43\, \mathrm{GHz}$ (trianlges) and the  Blandford-Znajek case at $15\, \mathrm{GHz}$ (squares) and $43\, \mathrm{GHz}$ (rhombus); \textbf{Cyan}: BL Lac for a conical geometry in the Eddington field case at $15\, \mathrm{GHz}$ (crosses) and $43\, \mathrm{GHz}$ (trianlges) and the  Blandford-Znajek case at $15\, \mathrm{GHz}$ (squares) and $43\, \mathrm{GHz}$ (rhombus); \textbf{Red}: FSRQs for the measured geometry in the Eddington field case at $15\, \mathrm{GHz}$ (crosses) and $43\, \mathrm{GHz}$ (trianlges) and the  Blandford-Znajek case at $15\, \mathrm{GHz}$ (squares) and $43\, \mathrm{GHz}$ (rhombus); \textbf{Orange}: FSRQs for a conical geometry in the Eddington field case at $15\, \mathrm{GHz}$ (crosses) and $43\, \mathrm{GHz}$ (trianlges) and the  Blandford-Znajek case at $15\, \mathrm{GHz}$ (squares) and $43\, \mathrm{GHz}$ (rhombus); \textbf{Green}: RGs for the measured geometry in the Eddington field case at $15\, \mathrm{GHz}$ (crosses) and $43\, \mathrm{GHz}$ (trianlges) and the  Blandford-Znajek case at $15\, \mathrm{GHz}$ (squares) and $43\, \mathrm{GHz}$ (rhombus); \textbf{Yellowgreen}: RGs for a conical geometry in the Eddington field case at $15\, \mathrm{GHz}$ (crosses) and $43\, \mathrm{GHz}$ (trianlges) and the  Blandford-Znajek case at $15\, \mathrm{GHz}$ (squares) and $43\, \mathrm{GHz}$ (rhombus);
      \textbf{Note}:In this plot, sources with guessed black hole masses ($\mathrm{log}\left(\frac{M}{M_{\odot}}\right)=8.77$) are shown.}
       \label{B_edd_plots}
\end{figure}

\begin{figure}
\centering
  %\includegraphics[width=\hsize]{./B_edd_plots/B_sc_tot.pdf}
  \includegraphics[width=\hsize]{./B_edd_plots/B_sc_tot_BHM_filtered.pdf}
  %\includegraphics[width=\hsize]{./B_edd_plots/B_sc_schwarzschild.pdf}
  %\includegraphics[width=\hsize]{./B_edd_plots/B_sc_retr.pdf}
      \caption{For a descriptoin of the general plots, see Fig.\ref{B_edd_plots}; \textbf{Note}:In this plot, sources with guessed black hole masses ($\mathrm{log}\left(\frac{M}{M_{\odot}}\right)=8.77$) are \textbf{not} shown. Here the RGs vanish from the plot (green and yeelowgreen datapoints) as well as some BL Lacs in the region $d\sim 10r_g$. Here as KS test was performed to test whether the FSRQs and the BL Lacs have the same underlying cumulative distribution function. In the case of the measured jet geometry, the KS test yields a  difference between the CFD of $\sim 0.74$ with a p-value of $\sim 2.7\times 10^{-5}$ in the case of a conical jet geometry the KS test yields: $d_{CDF}\sim 0.76\; ,p\sim 1.6\times 10^{-5}$. For both cases the KS test suggests that FSRQs and BL Lacs are drawn from a different distribution function, suggesting a systematic difference between those classes.}
      \label{B_edd_plots2}
\end{figure}




\begin{figure}
\centering
  \includegraphics[width=\hsize]{./B_edd_plots/B_sc_tot_BHM_filtered_pysical.pdf}
      \caption{See Fig.\ref{B_edd_plots} for a description, howevere here only sources with measured black hole masses as well as Scenarios which we consider as physical reasonable, are shown}
      \label{B_edd_physical}
\end{figure}



%cf. \citet{blandford_znajek}, \citet{daly2011}, \citet{daly2009} , \citet{daly2014} 
%\begin{equation}
%B_{BZ} \sim 10^4 \, \left( \frac{P_j}{10^{44}}\right)^{0.5} \left(\frac{M}{10^8}\right)^{-1} \frac{\sqrt{5}}{j} [G]
%\end{equation}
%where $P_j$ is the jet power, $M$ is the blck hole's mass and $j$ the spin of the black hole.

%In the following, maximum spinning black hole ($j=1$) are assumed. With this of course no absoluteb position scaling is found, however relative differences within the source classes can be studied. 


%The jet powers are obtained by estimating the power budget of theextended emission in the manner of \citet{godfrey2013}. For this the luminosities of the extended, unbeamed emission is obtained for each of the sources from \citet{Kharb2010}. 
%The jet powers, under the assumption, FSRQs can be assciated with rotated FR2 galaxies and BL Lacs with FR1 galaxies, can be estimated according to 
%\begin{equation}
%\begin{gathered}
%P_{j,\mathrm{FSRQs}} = 3 \times 10^{44} \left(\frac{L_{151}}{10^{25}}\right)^{0.67} \, W \\
%P_{j,\mathrm{BLLacs}} = 5 \times 10^{44} \left(\frac{L_{151}}{10^{25}}\right)^{0.64} \, W
%\end{gathered}
%\end{equation}
%In \citet{Kharb2010}, the luminositeis are measured at $1.4\,\mathrm{GHz}$, the method from \citet{godfrey2013} measures at $0.151\,\mathrm{GHz}$, therefore the Flux is sacled to the needed frequency with a power law of $\alpha \sim -0.75$ due to the spectrum of the extended, unbeamed emission of blazars at these frequencies. 

% With the magnetic field in the radio core and the magnetic frield from the Blandford-Znajek relation, and under the assumption that the Blandford-Znajek field is reached one gravitational radius $R_g$ from the jet engine, along the jet axis, the distance between the radfio core and the location of the blandford-Znajek field can be calculated according to  
%\begin{equation}
%d_{B_x,B_{BZ}} = \left(\frac{B_x}{1R_g ^b}\right) \times r^b \, .
%\end{equation}

%\begin{equation}
%j = \frac{a}{M} = \frac{\frac{S}{M\,c}}{\frac{G\,M}{c^2}}
%\end{equation}

%\begin{table*}
%\caption{\textbf{col.1}: name and class; \textbf{col.2}: black hole mass; \textbf{col.3}: estimated jet powers from the extended unbeamed emission; \textbf{col.4}: distance of the $15\,\mathrm{GHz}$ radio core to the point along the jet axis where the $15\,\mathrm{GHz}$ and $43\,\mathrm{GHz}$ jet have the same diameter; \textbf{col.5}: see col.4; \textbf{col.6}: magnetic field in the $15\,\mathrm{GHz}$ radio core; \textbf{col.7}: magnetic field in the $43\,\mathrm{GHz}$ radio core; \textbf{col.8}: scaled magnetic field at $15\,\mathrm{GHz}$ and a scaling according to equipartition; \textbf{col.9}: scaled magnetic field at $15\,\mathrm{GHz}$ and a scaling according to particle conservation; \textbf{col.10}: see col.8 at $43\,\mathrm{GHz}$; \textbf{col. 11}: see col.9 at $43\,\mathrm{GHz}$}
%\label{tab_B}
%\begin{tabular}{lcccccccccc}
%\toprule
%B1950, class& $\mathrm{log}\left(\frac{M}{M_{\odot}}\right)$& $P_j\, \frac{\mathrm{erg}}{s}$&$r_{15}/r_g$ &$r_{43}/r_g$ & $B_{c,15}/G$ &$B_{c,43}/G$ & $B' _{eq,15}/G$ & $B' _{pc,15}/G$ & $B' _{eq,43}/G $& $B' _{pc,43}/G$ \\
%\midrule
%0219+428 B & 8.77 & 2.16E+45 & 8.60E+03 & 1.38E+03 & 1.77 & 1.46 & 9.13E+02 & 1.37E+03 & 7.06E+01 & 5.09E+01 \\ \midrule
%0336-019 Q & 8.78 & 8.21E+46 & 2.72E+03 & 1.71E+03 & 0.69 & 1.2 & 3.39E+01 & 1.69E+01 & 3.17E+02 & 3.91E+02 \\ \midrule
%0415+379 G & 8.77 & 3.15E+46 & 2.58E+03 & 5.32E+02 & 3.33 & 3.36 & 4.69E+02 & 5.13E+02 & 1.36E+02 & 1.36E+02 \\ \midrule
%0430+052 G & 8.77 & 2.78E+45 & 8.09E+02 & 3.39E+02 & 1.99 & 3.88 & 9.65E+01 & 7.62E+01 & 1.09E+02 & 1.54E+02 \\ \midrule
%0528+134 Q & 8.77 & 1.73E+47 & 1.12E+04 & 1.45E+03 & 0.71 & 1.49 & 4.06E+02 & 3.46E+02 & 3.93E+01 & 1.89E+01 \\ \midrule
%0716+714 B & 8.77 & 3.74E+46 & 2.92E+03 & 9.88E+02 & - & - & - & - & - & - \\ \midrule
%0735+178 B & 8.77 & 2.58E+46 & 2.57E+03 & 9.57E+02 & - & - & - & - & - & - \\ \midrule
%0827+243 Q & 8.77 & 8.84E+46 & 1.15E+04 & 1.88E+03 & 1.01 & 1.17 & 5.86E+03 & 4.01E+04 & 2.62E+02 & 1.74E+03 \\ \midrule
%0829+046 B & 8.49 & 3.04E+46 & 2.27E+03 & 1.72E+03 & 0.97 & 1.42 & 3.77E+02 & 2.98E+02 & 2.19E+02 & 1.25E+02 \\ \midrule
%0836+710 Q & 9.49 & 2.11E+47 & 4.53E+02 & 1.91E+02 & 0.82 & 1.13 & 1.63E+02 & 1.53E+02 & 1.76E+01 & 2.37E+01 \\ \midrule
%0851+202 B & 8.77 & 1.14E+46 & 1.88E+03 & 1.83E+03 & 1.86 & 1.97 & 2.15E+03 & 3.89E+04 & 4.19E+04 & 7.70E+05 \\ \midrule
%0954+658 B & 8.77 & 2.16E+45 & 7.88E+03 & 1.28E+03 & - & - & - & - & - & - \\ \midrule
%1101+384 B & 8.77 & 2.16E+45 & 2.31E+02 & 8.68E+01 & - & - & - & - & - & - \\ \midrule
%1127-145 Q & 9.18 & 1.05E+47 & 1.83E+03 & 1.20E+03 & 0.49 & 0.92 & 7.22E+00 & 7.31E+00 & 2.64E+01 & 2.55E+01 \\ \midrule
%1156+295 Q & 9.19 & 1.45E+47 & 1.03E+03 & 1.05E+03 & 1.3 & 2.04 & 6.54E+02 & 8.42E+03 & 2.16E+02 & 6.56E+02 \\ \midrule
%1219+285 B & 8.77 & 2.16E+45 & 1.77E+03 & 2.18E+03 & 2.07 & 2.0 & 3.08E+03 & 5.97E+03 & 1.24E+02 & 1.36E+02 \\ \midrule
%1222+216 Q & 8.77 & 2.26E+47 & 5.98E+03 & 4.69E+03 & 2.52 & 2.27 & 6.39E+04 & 3.63E+05 & 5.84E+03 & 5.31E+04 \\ \midrule
%1226+023 Q & 8.76 & 4.69E+47 & 2.60E+03 & 3.23E+03 & 0.89 & 1.8 & 6.17E+01 & 2.00E+01 & 5.79E+01 & 5.01E+01 \\ \midrule
%1253-055 Q & 8.53 & 6.18E+47 & 1.51E+04 & 3.25E+03 & 0.99 & 1.22 & 1.51E+04 & 5.26E+04 & 1.01E+03 & 6.89E+03 \\ \midrule
%1308+326 Q & 8.77 & 9.52E+46 & 5.89E+03 & 2.86E+03 & 1.46 & 1.47 & 4.90E+03 & 7.53E+04 & 2.48E+03 & 7.92E+03 \\ \midrule
%1633+382 Q & 10.14 & 1.04E+47 & 3.51E+02 & 5.84E+01 & 1.37 & 2.01 & 4.90E+01 & 4.51E+01 & 3.26E+01 & 2.40E+01 \\ \midrule
%1652+398 B & 8.77 & 2.16E+45 & 1.94E+02 & 2.82E+02 & - & - & - & - & - & - \\ \midrule
%1730-130 Q & 8.77 & 3.36E+47 & 9.88E+03 & 4.52E+03 & 1.23 & 1.38 & 5.10E+03 & 1.12E+04 & 3.43E+03 & 8.46E+03 \\ \midrule
%1749+096 B & 8.34 & 7.19E+45 & 3.97E+03 & 4.39E+03 & 1.78 & 1.69 & 6.28E+04 & 2.29E+06 & 5.17E+03 & 3.91E+05 \\ \midrule
%2200+420 B & 8.42 & 2.16E+45 & 1.36E+04 & 1.88E+03 & 14.78 & 4.59 & 4.75E+04 & 4.67E+04 & 4.17E+03 & 3.40E+03 \\ \midrule
%2223-052 Q & 8.54 & 1.61E+47 & 2.18E+04 & 6.97E+03 & 0.58 & 0.69 & 2.81E+03 & 5.38E+03 & 5.63E+02 & 1.67E+03 \\ \midrule
%2230+114 Q & 8.64 & 1.65E+47 & 4.15E+03 & 2.55E+03 & 0.75 & 1.0 & 1.14E+02 & 8.82E+01 & 7.70E+01 & 1.00E+02 \\ \midrule
%2251+158 Q & 8.87 & 4.30E+47 & 2.37E+03 & 1.71E+03 & 0.51 & 0.99 & 3.43E+02 & 3.50E+02 & 7.29E+01 & 2.20E+02 \\ \bottomrule
%\end{tabular}
%\end{table*}













==> table_result.tex <==
%\begin{table*}
%\caption{\mk{\sout{The considered sources are listed;} Tables have only a short descriptive title: what is listed? The information about the column content goes into the table footer. You do not have to repeat what is already written in the column name. Here, the main information needed is why there are two entries in column 4 and 6 for each source. All abbreviations need to be introduced, unless they are given by the journal (e.g., Sect. or Fig.); Use longtab for tables longer than one page; Read the A\&A guide for authors.}; The new suggested Table 8 below is an example to format all fitting results in one table\\
%col. 1: \mk{B1915 $\rightarrow$ B\,1950} name (common name); col. 2: classification; col. 3: redshift, col. 4: diameter gradient (jet axis), col.5: $\chi ^2 _{\mathrm{red,l}}$ , slope; col. 6: $t_b$ gradient slope, col. 7: $\chi ^2 _{\mathrm{red,s}}$}
%\label{tab1a}
%\begin{tabular}{lcccccc}
%\toprule
%B1950 name  (Common name) & Classification & z & l & $\chi ^2 _{\mathrm{red,l}}$ & s & $\chi ^2 _{\mathrm{red,s}}$  \\
%\midrule
%0219+428 (3C 66A) & B & 0.34\tablefootmark{a} & $1.019 \pm 0.166$ & $0.99$ & $-2.047 \pm 0.427$ & $2.138$ \\ & & & $0.568 \pm 0.164$ & $0.932$ & $-1.598 \pm 0.354$ & $1.056$ \\ \midrule
%0336-019 (CTA 26) & Q & 0.852\tablefootmark{b} & $0.699 \pm 0.175$ & $3.508$ & $-1.119 \pm 0.382$ & $3.812$ \\ & & & $0.81 \pm 0.251$ & $2.653$ & $-1.872 \pm 0.476$ & $3.149$ \\ \midrule
%0415+379 (3C111) & G & 0.0491\tablefootmark{c} & $0.617 \pm 0.191$ & $2.526$ & $-1.834 \pm 0.591$ & $5.328$ \\ & & & $0.529 \pm 0.197$ & $1.224$ & $-1.512 \pm 0.549$ & $2.496$ \\ \midrule
%0430+052 (3C 120) & G & 0.033\tablefootmark{d} & $0.555 \pm 0.232$ & $5.571$ & $-1.542 \pm 0.539$ & $6.496$ \\ & & & $0.455 \pm 0.173$ & $1.033$ & $-1.674 \pm 0.477$ & $2.273$ \\ \midrule
%0528+134 (PKS 0528+134) & Q & 2.07\tablefootmark{e} & $0.792 \pm 0.209$ & $1.836$ & $-2.646 \pm 0.458$ & $2.527$ \\ & & & $0.448 \pm 0.19$ & $1.497$ & $-1.226 \pm 0.429$ & $2.417$ \\ \midrule
%0716+714 (TXS 0716+714) & B & 0.803\tablefootmark{f} & $0.845 \pm 0.156$ & $0.571$ & $-2.997 \pm 0.35$ & $0.295$ \\ & & & $0.781 \pm 0.208$ & $1.842$ & $-2.596 \pm 0.523$ & $1.023$ \\ \midrule
%0735+178 (OI 158) & B & 0.45\tablefootmark{g} & $0.854 \pm 0.08$ & $0.612$ & $-2.457 \pm 0.372$ & $2.294$ \\ & & & $0.767 \pm 0.21$ & $1.177$ & $-1.753 \pm 0.365$ & $0.958$ \\ \midrule
%0827+243 (OJ 248) & Q & 0.94\tablefootmark{h} & $0.818 \pm 0.193$ & $1.15$ & $-2.606 \pm 0.472$ & $1.617$ \\ & & & $0.557 \pm 0.171$ & $0.691$ & $-2.546 \pm 0.485$ & $1.613$ \\ \midrule
%0829+046 (OJ 049) & B & 0.174\tablefootmark{i} & $0.975 \pm 0.131$ & $0.965$ & $-2.565 \pm 0.304$ & $0.913$ \\ & & & $0.697 \pm 0.234$ & $1.663$ & $-1.873 \pm 0.538$ & $1.81$ \\ \midrule
%0836+710 (4C +71.07) & Q & 0.69\tablefootmark{j} & $0.768 \pm 0.18$ & $2.665$ & $-1.963 \pm 0.491$ & $14.188$ \\ & & & $0.367 \pm 0.224$ & $3.854$ & $-1.965 \pm 0.7$ & $15.779$ \\ \midrule
%0851+202 (OJ 287) & B & 0.306\tablefootmark{k} & $0.875 \pm 0.187$ & $1.518$ & $-2.869 \pm 0.459$ & $2.885$ \\ & & & $0.823 \pm 0.336$ & $5.126$ & $-2.79 \pm 0.81$ & $8.322$ \\ \midrule
%0954+658 (S4 0954+65) & B & 0.45\tablefootmark{l} & $1.195 \pm 0.211$ & $1.163$ & $-3.392 \pm 0.473$ & $1.321$ \\ & & & $1.092 \pm 0.251$ & $2.761$ & $-2.97 \pm 0.524$ & $2.4$ \\ \midrule
%1101+384 (Mrk 421) & B & 0.0308\tablefootmark{m} & $0.891 \pm 0.185$ & $1.782$ & $-2.195 \pm 0.257$ & $0.866$ \\ & & & $0.611 \pm 0.263$ & $1.905$ & $-1.571 \pm 0.458$ & $1.547$ \\ \midrule
%1127-145 (PKS 1127-14) & Q & 1.184\tablefootmark{n} & $0.48 \pm 0.242$ & $6.303$ & $-1.141 \pm 0.664$ & $10.694$ \\ & & & $0.351 \pm 0.259$ & $7.136$ & $-1.519 \pm 0.624$ & $6.062$ \\ \midrule
%1156+295 (4C +29.45) & Q & 0.725\tablefootmark{i} & $0.759 \pm 0.163$ & $3.577$ & $-2.473 \pm 0.385$ & $1.055$ \\ & & & $0.728 \pm 0.176$ & $1.557$ & $-2.235 \pm 0.493$ & $2.48$ \\ \midrule
%1219+285 (W Comae) & B & 0.102\tablefootmark{o} & $0.775 \pm 0.201$ & $2.054$ & $-1.779 \pm 0.382$ & $1.269$ \\ & & & $0.733 \pm 0.232$ & $1.342$ & $-1.756 \pm 0.502$ & $1.905$ \\ \midrule
%1222+216 (4C +21.35) & Q & 0.433\tablefootmark{i} & $0.853 \pm 0.186$ & $2.216$ & $-2.174 \pm 0.583$ & $3.47$ \\ & & & $0.547 \pm 0.173$ & $0.736$ & $-2.505 \pm 0.583$ & $2.292$ \\ \midrule
%1226+023 (3C 273) & Q & 0.1583\tablefootmark{p} & $0.682 \pm 0.209$ & $12.906$ & $-1.857 \pm 0.47$ & $9.143$ \\ & & & $0.501 \pm 0.23$ & $4.716$ & $-1.651 \pm 0.473$ & $3.594$ \\ \midrule
%1253-055 (3C 279) & Q & 0.6\tablefootmark{q} & $0.85 \pm 0.303$ & $10.057$ & $-2.327 \pm 0.634$ & $9.179$ \\ & & & $0.436 \pm 0.244$ & $3.698$ & $-1.952 \pm 0.694$ & $4.586$ \\ \midrule
%1308+326 (OP 313) & Q & 0.997\tablefootmark{i} & $0.897 \pm 0.253$ & $2.794$ & $-2.577 \pm 0.607$ & $3.602$ \\ & & & $0.865 \pm 0.25$ & $2.625$ & $-2.808 \pm 0.661$ & $3.67$ \\ \midrule
%1633+382 (4C +38.41) & Q & 1.814\tablefootmark{h} & $0.736 \pm 0.22$ & $4.757$ & $-2.16 \pm 0.473$ & $5.26$ \\ & & & $0.705 \pm 0.223$ & $2.857$ & $-1.901 \pm 0.45$ & $4.236$ \\
%\bottomrule 
%\end{tabular}
%\tablefoot{ \\
%\tablefoottext{a}{\citet{0219+428}}
%\tablefoottext{b}{\citet{0336-019}}
%\tablefoottext{c}{\citet{0415+379}}
%\tablefoottext{d}{\citet{0430+052}} \\
%\tablefoottext{e}{\citet{0528+134}}
%\tablefoottext{f}{\citet{0716+714}}
%\tablefoottext{g}{\citet{0735+178}}
%\tablefoottext{h}{\citet{Paris2017}}
%\tablefoottext{i}{\citet{Schneider2010}} \\
%\tablefoottext{j}{\citet{0836+710}}
%\tablefoottext{k}{\citet{0851+202}}
%\tablefoottext{l}{\citet{0954+658}}
%\tablefoottext{m}{\citet{1101+384}}
%\tablefoottext{n}{\citet{1127-145}} \\
%\tablefoottext{o}{\citet{1219+285}}
%\tablefoottext{p}{\citet{1226+023}}
%\tablefoottext{q}{\citet{1253-055}}
%}
%\end{table*}

%\begin{table*}
%\caption{Tab. \ref{tab1a} continuation; col. 1: B1915 name (common name); col. 2: classification; col. 3: redshift, col. 4: diameter gradient (jet axis), col.5: $\chi ^2 %_{\mathrm{red,l}}$ , slope; col. 6: $t_b$ gradient slope, col. 7: $\chi ^2 _{\mathrm{red,s}}$}
%\label{tab1b}
%\begin{tabular}{lcccccc}
%\toprule
%B1950 name  (Common name) & Classification & z & l & $\chi ^2 _{\mathrm{red,l}}$ & s & $\chi ^2 _{\mathrm{red,s}}$  \\
%\midrule
%1652+398 (Mrk 501) & B & 0.0337\tablefootmark{r} & $0.639 \pm 0.137$ & $6.53$ & $-1.719 \pm 0.184$ & $1.169$ \\ & & & $0.508 \pm 0.219$ & $1.361$ & $-1.329 \pm 0.394$ & $1.957$ %\\ \midrule
%1730-130 (NRAO 530) & Q & 0.902\tablefootmark{s} & $0.678 \pm 0.197$ & $9.439$ & $-1.632 \pm 0.458$ & $6.527$ \\ & & & $1.043 \pm 0.265$ & $2.832$ & $-2.783 \pm 0.484$ & $2.936$ \\ \midrule
%1749+096 (OT 081) & B & 0.322\tablefootmark{t} & $0.983 \pm 0.163$ & $0.889$ & $-3.099 \pm 0.341$ & $1.049$ \\ & & & $0.792 \pm 0.26$ & $2.463$ & $-3.191 \pm 0.636$ & $3.675$ \\ \midrule
%2200+420 (BL Lac) & B & 0.0686\tablefootmark{u} & $1.594 \pm 0.302$ & $5.072$ & $-2.979 \pm 0.456$ & $5.951$ \\ & & & $0.844 \pm 0.183$ & $3.443$ & $-2.399 \pm 0.494$ & $3.582$ \\ \midrule
%2223-052 (3C 446) & Q & 1.404\tablefootmark{v} & $0.605 \pm 0.238$ & $2.759$ & $-2.492 \pm 0.417$ & $2.533$ \\ & & & $0.89 \pm 0.235$ & $2.51$ & $-2.45 \pm 0.449$ & $3.7$ \\ \midrule
%2230+114 (CTA 102) & Q & 1.037\tablefootmark{w} & $0.763 \pm 0.234$ & $6.77$ & $-1.912 \pm 0.412$ & $4.347$ \\ & & & $0.578 \pm 0.26$ & $2.298$ & $-1.7 \pm 0.534$ & $2.535$ \\ \midrule
%2251+158 (3C 454.3) & Q & 0.859\tablefootmark{x} & $0.772 \pm 0.2$ & $13.612$ & $-1.942 \pm 0.388$ & $8.279$ \\ & & & $0.484 \pm 0.261$ & $3.55$ & $-1.963 \pm 0.631$ & $5.477$ \\ 
%\bottomrule 
%\end{tabular}
%\tablefoot{ \\
%\tablefoottext{r}{\citet{1652+398}}
%\tablefoottext{s}{\citet{1730-130}} \\
%\tablefoottext{t}{\citet{1749+096}}
%\tablefoottext{u}{\citet{2200+420}}
%\tablefoottext{v}{\citet{2223-052}}
%\tablefoottext{w}{\citet{2230+114}}
%\tablefoottext{x}{\citet{2251+158}}
%}
%\end{table*}


%\begin{table*}
%\caption{The considered sources are listed; col. 1: B1915 name (common name); col. 2: classification , col. 3: diameter gradient (jet axis) in the voerlap region of the 15 GHz and 43 GHz jets, col.4: $\chi ^2 _{\mathrm{red,l}}$ , slope; col. 5: $t_b$ gradient slope in the voerlap region of the 15 GHz and 43 GHz jets, col. 6: $\chi ^2 _{\mathrm{red,s}}$}
%\label{tab2a}
%\begin{tabular}{lccccc}
%\toprule
%B1950 name  (Common name) & Classification & $l_{\mathrm{overlap}}$ & $\chi ^2 _{\mathrm{red,l,overlap}}$ & $s_{\mathrm{overlap}}$ & $\chi ^2 _{\mathrm{red,s,overlap}}$  \\
%\midrule
%0219+428 (3C 66A) & B & $0.635 \pm 0.12$ & $0.415$ & $-2.077 \pm 0.385$ & $1.094$ \\ & &  $0.561 \pm 0.17$ & $1.07$ & $-1.453 \pm 0.36$ & $1.172$ \\ \midrule
%0336-019 (CTA 26) & Q & $0.678 \pm 0.184$ & $3.897$ & $-1.176 \pm 0.359$ & $3.132$ \\ & &  $0.84 \pm 0.263$ & $3.003$ & $-1.703 \pm 0.51$ & $3.612$ \\ \midrule
%0415+379 (3C111) & G & $0.577 \pm 0.202$ & $2.84$ & $-1.571 \pm 0.626$ & $5.968$ \\ & &  $0.597 \pm 0.181$ & $1.257$ & $-1.564 \pm 0.534$ & $2.675$ \\ \midrule
%0430+052 (3C 120) & G & $0.556 \pm 0.193$ & $2.99$ & $-1.415 \pm 0.542$ & $5.003$ \\ & &  $0.433 \pm 0.181$ & $1.189$ & $-1.437 \pm 0.506$ & $2.54$ \\ \midrule
%0528+134 (PKS 0528+134) & Q & $0.6 \pm 0.178$ & $1.837$ & $-2.336 \pm 0.587$ & $4.496$ \\ & &  $0.512 \pm 0.187$ & $1.531$ & $-1.944 \pm 0.426$ & $2.429$ \\ \midrule
%0716+714 (TXS 0716+714) & B & $0.792 \pm 0.143$ & $0.608$ & $-2.841 \pm 0.354$ & $0.346$ \\ & &  $0.78 \pm 0.188$ & $1.474$ & $-2.563 \pm 0.46$ & $0.745$ \\ \midrule
%0735+178 (OI 158) & B & $0.834 \pm 0.085$ & $0.67$ & $-1.846 \pm 0.325$ & $1.628$ \\ & &  $0.752 \pm 0.207$ & $1.236$ & $-1.772 \pm 0.294$ & $0.761$ \\ \midrule
%0827+243 (OJ 248) & Q & $0.832 \pm 0.174$ & $0.994$ & $-3.108 \pm 0.504$ & $2.204$ \\ & &  $0.54 \pm 0.137$ & $0.598$ & $-2.74 \pm 0.438$ & $1.388$ \\ \midrule
%0829+046 (OJ 049) & B & $0.696 \pm 0.123$ & $0.553$ & $-1.999 \pm 0.335$ & $0.883$ \\ & &  $0.788 \pm 0.241$ & $1.759$ & $-1.894 \pm 0.563$ & $1.993$ \\ \midrule
%0836+710 (4C +71.07) & Q & $0.459 \pm 0.182$ & $1.167$ & $-1.985 \pm 0.523$ & $14.09$ \\ & &  $0.297 \pm 0.221$ & $4.652$ & $-1.626 \pm 0.664$ & $15.912$ \\ \midrule
%0851+202 (OJ 287) & B & $0.694 \pm 0.175$ & $1.313$ & $-2.096 \pm 0.493$ & $2.972$ \\ & &  $0.94 \pm 0.327$ & $5.72$ & $-3.046 \pm 0.765$ & $8.676$ \\ \midrule
%0954+658 (S4 0954+65) & B & $1.37 \pm 0.209$ & $1.216$ & $-3.978 \pm 0.499$ & $1.563$ \\ & &  $1.165 \pm 0.257$ & $3.134$ & $-3.316 \pm 0.524$ & $2.748$ \\ \midrule
%1101+384 (Mrk 421) & B & $0.752 \pm 0.147$ & $1.899$ & $-2.2 \pm 0.197$ & $1.07$ \\ & &  $0.65 \pm 0.273$ & $2.038$ & $-1.568 \pm 0.446$ & $1.545$ \\ \midrule
%1127-145 (PKS 1127-14) & Q & $0.409 \pm 0.272$ & $7.479$ & $-1.033 \pm 0.611$ & $9.153$ \\ & &  $0.707 \pm 0.249$ & $5.821$ & $-2.182 \pm 0.596$ & $6.137$ \\ \midrule
%1156+295 (4C +29.45) & Q & $0.551 \pm 0.141$ & $0.523$ & $-2.205 \pm 0.468$ & $1.421$ \\ & &  $0.727 \pm 0.179$ & $1.621$ & $-2.436 \pm 0.492$ & $2.652$ \\ \midrule
%1219+285 (W Comae) & B & $0.976 \pm 0.178$ & $0.769$ & $-2.582 \pm 0.323$ & $0.501$ \\ & &  $0.737 \pm 0.259$ & $1.73$ & $-1.563 \pm 0.52$ & $2.166$ \\ \midrule
%1222+216 (4C +21.35) & Q & $0.928 \pm 0.139$ & $0.382$ & $-3.467 \pm 0.523$ & $2.122$ \\ & &  $0.528 \pm 0.177$ & $0.824$ & $-2.894 \pm 0.606$ & $2.716$ \\ \midrule
%1226+023 (3C 273) & Q & $0.81 \pm 0.239$ & $9.064$ & $-1.932 \pm 0.498$ & $6.806$ \\ & &  $0.485 \pm 0.235$ & $5.223$ & $-1.634 \pm 0.465$ & $3.759$ \\ \midrule
%1253-055 (3C 279) & Q & $0.922 \pm 0.219$ & $3.98$ & $-2.96 \pm 0.5$ & $4.173$ \\ & &  $0.599 \pm 0.239$ & $3.637$ & $-2.529 \pm 0.685$ & $4.335$ \\ \midrule
%1308+326 (OP 313) & Q & $0.694 \pm 0.21$ & $1.886$ & $-2.881 \pm 0.558$ & $3.117$ \\ & &  $0.865 \pm 0.25$ & $2.625$ & $-2.808 \pm 0.661$ & $3.67$ \\ \midrule
%1633+382 (4C +38.41) & Q & $0.747 \pm 0.231$ & $5.18$ & $-1.841 \pm 0.492$ & $7.078$ \\ & &  $0.716 \pm 0.223$ & $3.04$ & $-1.92 \pm 0.441$ & $4.637$ \\ 
%\bottomrule 
%\end{tabular}
%\end{table*}

%\begin{table*}
%\caption{continuation of Tab.\ref{tab2a}; col. 1: B1915 name (common name); col. 2: classification , col. 3: diameter gradient (jet axis) in the voerlap region of the 15 GHz and 43 GHz jets, col.4: $\chi ^2 _{\mathrm{red,l}}$ , slope; col. 5: $t_b$ gradient slope in the voerlap region of the 15 GHz and 43 GHz jets, col. 6: $\chi ^2 _{\mathrm{red,s}}$}
%\label{tab2b}
%\begin{tabular}{lccccc}
%\toprule
%B1950 name  (Common name) & Classification & $l_{\mathrm{overlap}}$ & $\chi ^2 _{\mathrm{red,l,overlap}}$ & $s_{\mathrm{overlap}}$ & $\chi ^2 _{\mathrm{red,s,overlap}}$  \\
%\midrule
%1652+398 (Mrk 501) & B & $0.531 \pm 0.153$ & $0.598$ & $-1.372 \pm 0.167$ & $0.31$ \\ & &  $0.807 \pm 0.164$ & $0.791$ & $-1.511 \pm 0.165$ & $0.356$ \\ \midrule
%1730-130 (NRAO 530) & Q & $0.854 \pm 0.214$ & $5.767$ & $-2.638 \pm 0.393$ & $3.739$ \\ & &  $1.052 \pm 0.256$ & $2.853$ & $-2.794 \pm 0.439$ & $2.786$ \\ \midrule
%1749+096 (OT 081) & B & $0.985 \pm 0.173$ & $0.966$ & $-3.337 \pm 0.375$ & $1.229$ \\ & &  $0.95 \pm 0.27$ & $2.462$ & $-3.467 \pm 0.542$ & $2.595$ \\ \midrule
%2200+420 (BL Lac) & B & $0.912 \pm 0.171$ & $3.598$ & $-2.447 \pm 0.404$ & $3.502$ \\ & &  $0.956 \pm 0.17$ & $3.154$ & $-2.583 \pm 0.456$ & $3.536$ \\ \midrule
%2223-052 (3C 446) & Q & $0.629 \pm 0.251$ & $3.705$ & $-2.747 \pm 0.476$ & $3.812$ \\ & &  $0.957 \pm 0.233$ & $2.347$ & $-2.441 \pm 0.414$ & $3.198$ \\ \midrule
%2230+114 (CTA 102) & Q & $0.708 \pm 0.134$ & $1.218$ & $-2.484 \pm 0.354$ & $2.135$ \\ & &  $0.686 \pm 0.269$ & $2.788$ & $-1.834 \pm 0.537$ & $2.756$ \\ \midrule
%2251+158 (3C 454.3) & Q & $0.876 \pm 0.205$ & $9.712$ & $-2.461 \pm 0.404$ & $6.407$ \\ & &  $0.476 \pm 0.276$ & $3.994$ & $-1.753 \pm 0.667$ & $5.854$ \\ 
%\bottomrule 
%\end{tabular}
%\end{table*}





\begin{table*}

\caption{Fitting results of jet geometry and brightness-temperature gradients}
\label{tab-fitresults}
\centering
\resizebox{1.3\columnwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
Name & $l_{\mathrm{15}}$ & $l_{\mathrm{43}}$ & $s_{\mathrm{15}}$ & $s_{\mathrm{43}}$  \\
\midrule
0219+428 & $1.02 \pm 0.17$ $(1.0)$ & $0.57 \pm 0.16$ $(0.9)$ & $-2.05 \pm 0.43$ $(2.1) $ & $-1.6 \pm 0.35$ $(1.1)$\\ & $0.63 \pm 0.12$ $(0.4)$ & $0.56 \pm 0.17$ $(1.1)$ & $-2.08 \pm 0.38$ $(1.1) $ & $-1.45 \pm 0.36$ $(1.2)$\\ \midrule
0336-019 & $0.7 \pm 0.17$ $(3.5)$ & $0.81 \pm 0.25$ $(2.7)$ & $-1.12 \pm 0.38$ $(3.8) $ & $-1.87 \pm 0.48$ $(3.1)$\\ & $0.68 \pm 0.18$ $(3.9)$ & $0.84 \pm 0.26$ $(3.0)$ & $-1.18 \pm 0.36$ $(3.1) $ & $-1.7 \pm 0.51$ $(3.6)$\\ \midrule
0415+379 & $0.62 \pm 0.19$ $(2.5)$ & $0.53 \pm 0.2$ $(1.2)$ & $-1.83 \pm 0.59$ $(5.3) $ & $-1.51 \pm 0.55$ $(2.5)$\\ & $0.58 \pm 0.2$ $(2.8)$ & $0.6 \pm 0.18$ $(1.3)$ & $-1.57 \pm 0.63$ $(6.0) $ & $-1.56 \pm 0.53$ $(2.7)$\\ \midrule
0430+052 & $0.56 \pm 0.23$ $(5.6)$ & $0.46 \pm 0.17$ $(1.0)$ & $-1.54 \pm 0.54$ $(6.5) $ & $-1.67 \pm 0.48$ $(2.3)$\\ & $0.56 \pm 0.19$ $(3.0)$ & $0.43 \pm 0.18$ $(1.2)$ & $-1.42 \pm 0.54$ $(5.0) $ & $-1.44 \pm 0.51$ $(2.5)$\\ \midrule
0528+134 & $0.79 \pm 0.21$ $(1.8)$ & $0.45 \pm 0.19$ $(1.5)$ & $-2.65 \pm 0.46$ $(2.5) $ & $-1.23 \pm 0.43$ $(2.4)$\\ & $0.6 \pm 0.18$ $(1.8)$ & $0.51 \pm 0.19$ $(1.5)$ & $-2.34 \pm 0.59$ $(4.5) $ & $-1.94 \pm 0.43$ $(2.4)$\\ \midrule
0716+714 & $0.84 \pm 0.16$ $(0.6)$ & $0.78 \pm 0.21$ $(1.8)$ & $-3.0 \pm 0.35$ $(0.3) $ & $-2.6 \pm 0.52$ $(1.0)$\\ & $0.79 \pm 0.14$ $(0.6)$ & $0.78 \pm 0.19$ $(1.5)$ & $-2.84 \pm 0.35$ $(0.3) $ & $-2.56 \pm 0.46$ $(0.7)$\\ \midrule
0735+178 & $0.85 \pm 0.08$ $(0.6)$ & $0.77 \pm 0.21$ $(1.2)$ & $-2.46 \pm 0.37$ $(2.3) $ & $-1.75 \pm 0.36$ $(1.0)$\\ & $0.83 \pm 0.08$ $(0.7)$ & $0.75 \pm 0.21$ $(1.2)$ & $-1.85 \pm 0.33$ $(1.6) $ & $-1.77 \pm 0.29$ $(0.8)$\\ \midrule
0827+243 & $0.82 \pm 0.19$ $(1.2)$ & $0.56 \pm 0.17$ $(0.7)$ & $-2.61 \pm 0.47$ $(1.6) $ & $-2.55 \pm 0.48$ $(1.6)$\\ & $0.83 \pm 0.17$ $(1.0)$ & $0.54 \pm 0.14$ $(0.6)$ & $-3.11 \pm 0.5$ $(2.2) $ & $-2.74 \pm 0.44$ $(1.4)$\\ \midrule
0829+046 & $0.98 \pm 0.13$ $(1.0)$ & $0.7 \pm 0.23$ $(1.7)$ & $-2.56 \pm 0.3$ $(0.9) $ & $-1.87 \pm 0.54$ $(1.8)$\\ & $0.7 \pm 0.12$ $(0.6)$ & $0.79 \pm 0.24$ $(1.8)$ & $-2.0 \pm 0.33$ $(0.9) $ & $-1.89 \pm 0.56$ $(2.0)$\\ \midrule
0836+710 & $0.77 \pm 0.18$ $(2.7)$ & $0.37 \pm 0.22$ $(3.9)$ & $-1.96 \pm 0.49$ $(14.2) $ & $-1.97 \pm 0.7$ $(15.8)$\\ & $0.46 \pm 0.18$ $(1.2)$ & $0.3 \pm 0.22$ $(4.7)$ & $-1.98 \pm 0.52$ $(14.1) $ & $-1.63 \pm 0.66$ $(15.9)$\\ \midrule
0851+202 & $0.88 \pm 0.19$ $(1.5)$ & $0.82 \pm 0.34$ $(5.1)$ & $-2.87 \pm 0.46$ $(2.9) $ & $-2.79 \pm 0.81$ $(8.3)$\\ & $0.69 \pm 0.17$ $(1.3)$ & $0.94 \pm 0.33$ $(5.7)$ & $-2.1 \pm 0.49$ $(3.0) $ & $-3.05 \pm 0.77$ $(8.7)$\\ \midrule
0954+658 & $1.2 \pm 0.21$ $(1.2)$ & $1.09 \pm 0.25$ $(2.8)$ & $-3.39 \pm 0.47$ $(1.3) $ & $-2.97 \pm 0.52$ $(2.4)$\\ & $1.37 \pm 0.21$ $(1.2)$ & $1.17 \pm 0.26$ $(3.1)$ & $-3.98 \pm 0.5$ $(1.6) $ & $-3.32 \pm 0.52$ $(2.7)$\\ \midrule
1101+384 & $0.89 \pm 0.19$ $(1.8)$ & $0.61 \pm 0.26$ $(1.9)$ & $-2.19 \pm 0.26$ $(0.9) $ & $-1.57 \pm 0.46$ $(1.5)$\\ & $0.75 \pm 0.15$ $(1.9)$ & $0.65 \pm 0.27$ $(2.0)$ & $-2.2 \pm 0.2$ $(1.1) $ & $-1.57 \pm 0.45$ $(1.5)$\\ \midrule
1127-145 & $0.48 \pm 0.24$ $(6.3)$ & $0.35 \pm 0.26$ $(7.1)$ & $-1.14 \pm 0.66$ $(10.7) $ & $-1.52 \pm 0.62$ $(6.1)$\\ & $0.41 \pm 0.27$ $(7.5)$ & $0.71 \pm 0.25$ $(5.8)$ & $-1.03 \pm 0.61$ $(9.2) $ & $-2.18 \pm 0.6$ $(6.1)$\\ \midrule
1156+295 & $0.76 \pm 0.16$ $(3.6)$ & $0.73 \pm 0.18$ $(1.6)$ & $-2.47 \pm 0.39$ $(1.1) $ & $-2.24 \pm 0.49$ $(2.5)$\\ & $0.55 \pm 0.14$ $(0.5)$ & $0.73 \pm 0.18$ $(1.6)$ & $-2.21 \pm 0.47$ $(1.4) $ & $-2.44 \pm 0.49$ $(2.7)$\\ \midrule
1219+285 & $0.77 \pm 0.2$ $(2.1)$ & $0.73 \pm 0.23$ $(1.3)$ & $-1.78 \pm 0.38$ $(1.3) $ & $-1.76 \pm 0.5$ $(1.9)$\\ & $0.98 \pm 0.18$ $(0.8)$ & $0.74 \pm 0.26$ $(1.7)$ & $-2.58 \pm 0.32$ $(0.5) $ & $-1.56 \pm 0.52$ $(2.2)$\\ \midrule
1222+216 & $0.85 \pm 0.19$ $(2.2)$ & $0.55 \pm 0.17$ $(0.7)$ & $-2.17 \pm 0.58$ $(3.5) $ & $-2.5 \pm 0.58$ $(2.3)$\\ & $0.93 \pm 0.14$ $(0.4)$ & $0.53 \pm 0.18$ $(0.8)$ & $-3.47 \pm 0.52$ $(2.1) $ & $-2.89 \pm 0.61$ $(2.7)$\\ \midrule
1226+023 & $0.68 \pm 0.21$ $(12.9)$ & $0.5 \pm 0.23$ $(4.7)$ & $-1.86 \pm 0.47$ $(9.1) $ & $-1.65 \pm 0.47$ $(3.6)$\\ & $0.81 \pm 0.24$ $(9.1)$ & $0.48 \pm 0.23$ $(5.2)$ & $-1.93 \pm 0.5$ $(6.8) $ & $-1.63 \pm 0.46$ $(3.8)$\\ \midrule
1253-055 & $0.85 \pm 0.3$ $(10.1)$ & $0.44 \pm 0.24$ $(3.7)$ & $-2.33 \pm 0.63$ $(9.2) $ & $-1.95 \pm 0.69$ $(4.6)$\\ & $0.92 \pm 0.22$ $(4.0)$ & $0.6 \pm 0.24$ $(3.6)$ & $-2.96 \pm 0.5$ $(4.2) $ & $-2.53 \pm 0.69$ $(4.3)$\\ \midrule
1308+326 & $0.9 \pm 0.25$ $(2.8)$ & $0.87 \pm 0.25$ $(2.6)$ & $-2.58 \pm 0.61$ $(3.6) $ & $-2.81 \pm 0.66$ $(3.7)$\\ & $0.69 \pm 0.21$ $(1.9)$ & $0.87 \pm 0.25$ $(2.6)$ & $-2.88 \pm 0.56$ $(3.1) $ & $-2.81 \pm 0.66$ $(3.7)$\\ \midrule
1633+382 & $0.74 \pm 0.22$ $(4.8)$ & $0.71 \pm 0.22$ $(2.9)$ & $-2.16 \pm 0.47$ $(5.3) $ & $-1.9 \pm 0.45$ $(4.2)$\\ & $0.75 \pm 0.23$ $(5.2)$ & $0.72 \pm 0.22$ $(3.0)$ & $-1.84 \pm 0.49$ $(7.1) $ & $-1.92 \pm 0.44$ $(4.6)$\\ \midrule
1652+398 & $0.64 \pm 0.14$ $(6.5)$ & $0.51 \pm 0.22$ $(1.4)$ & $-1.72 \pm 0.18$ $(1.2) $ & $-1.33 \pm 0.39$ $(2.0)$\\ & $0.53 \pm 0.15$ $(0.6)$ & $0.81 \pm 0.16$ $(0.8)$ & $-1.37 \pm 0.17$ $(0.3) $ & $-1.51 \pm 0.16$ $(0.4)$\\ \midrule
1730-130 & $0.68 \pm 0.2$ $(9.4)$ & $1.04 \pm 0.26$ $(2.8)$ & $-1.63 \pm 0.46$ $(6.5) $ & $-2.78 \pm 0.48$ $(2.9)$\\ & $0.85 \pm 0.21$ $(5.8)$ & $1.05 \pm 0.26$ $(2.9)$ & $-2.64 \pm 0.39$ $(3.7) $ & $-2.79 \pm 0.44$ $(2.8)$\\ \midrule
1749+096 & $0.98 \pm 0.16$ $(0.9)$ & $0.79 \pm 0.26$ $(2.5)$ & $-3.1 \pm 0.34$ $(1.0) $ & $-3.19 \pm 0.64$ $(3.7)$\\ & $0.99 \pm 0.17$ $(1.0)$ & $0.95 \pm 0.27$ $(2.5)$ & $-3.34 \pm 0.38$ $(1.2) $ & $-3.47 \pm 0.54$ $(2.6)$\\ \midrule
2200+420 & $1.59 \pm 0.3$ $(5.1)$ & $0.84 \pm 0.18$ $(3.4)$ & $-2.98 \pm 0.46$ $(6.0) $ & $-2.4 \pm 0.49$ $(3.6)$\\ & $0.91 \pm 0.17$ $(3.6)$ & $0.96 \pm 0.17$ $(3.2)$ & $-2.45 \pm 0.4$ $(3.5) $ & $-2.58 \pm 0.46$ $(3.5)$\\ \midrule
2223-052 & $0.61 \pm 0.24$ $(2.8)$ & $0.89 \pm 0.24$ $(2.5)$ & $-2.49 \pm 0.42$ $(2.5) $ & $-2.45 \pm 0.45$ $(3.7)$\\ & $0.63 \pm 0.25$ $(3.7)$ & $0.96 \pm 0.23$ $(2.3)$ & $-2.75 \pm 0.48$ $(3.8) $ & $-2.44 \pm 0.41$ $(3.2)$\\ \midrule
2230+114 & $0.76 \pm 0.23$ $(6.8)$ & $0.58 \pm 0.26$ $(2.3)$ & $-1.91 \pm 0.41$ $(4.3) $ & $-1.7 \pm 0.53$ $(2.5)$\\ & $0.71 \pm 0.13$ $(1.2)$ & $0.69 \pm 0.27$ $(2.8)$ & $-2.48 \pm 0.35$ $(2.1) $ & $-1.83 \pm 0.54$ $(2.8)$\\ \midrule
2251+158 & $0.77 \pm 0.2$ $(13.6)$ & $0.48 \pm 0.26$ $(3.6)$ & $-1.94 \pm 0.39$ $(8.3) $ & $-1.96 \pm 0.63$ $(5.5)$\\ & $0.88 \pm 0.2$ $(9.7)$ & $0.48 \pm 0.28$ $(4.0)$ & $-2.46 \pm 0.4$ $(6.4) $ & $-1.75 \pm 0.67$ $(5.9)$\\ 
\bottomrule
\end{tabular}
}
\tablefoot{For each source, the top row refers to the full jet length probed and the bottom row refers to the overlap region probed at both frequencies; Columns: (1) IAU B\,1950 name, (2) Fit parameter of jet-geometry at 15\,GHz $l$ (reduced $\chi ^2$), (3) Fit parameter of jet-geometry at 43\,GHz $l$ (reduced $\chi ^2$), (4) Fit parameter of brightness-temperature gradient at 15\,GHz $l$ (reduced $\chi ^2$), (3) Fit parameter of brightness-temperature gradient at 43\,GHz $l$ (reduced $\chi ^2$) }

\end{table*}
